Generators and Relations for the Group On(Z[1/2])

We give a finite presentation by generators and relations for the group O_n(Z[1/2]) of n-dimensional orthogonal matrices with entries in Z[1/2]. We then obtain a similar presentation for the group of n-dimensional orthogonal matrices of the form M/sqrt(2)^k, where k is a nonnegative integer and M is an integer matrix. Both groups arise in the study of quantum circuits. In particular, when the dimension is a power of 2, the elements of the latter group are precisely the unitary matrices that can be represented by a quantum circuit over the universal gate set consisting of the Toffoli gate, the Hadamard gate, and the computational ancilla.

==> eptcsdata.tex <==
\providecommand{\firstpage}{210}
\providecommand{\publicationstatus}{M. Backens, C. Heunen (Eds.): Quantum Physics and Logic (QPL) 2021\\
EPTCS 343, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.343.11}{10.4204/EPTCS.343.11}}

